VOR-Bench: A Human Perception-Driven Benchmark for Video Object Removal

Despite its crucial role in video object removal (VOR), existing evaluation paradigms face two critical limitations: questionable references and a misalignment between tradi- tional metrics and human preference. To address these challenges, we introduce VOR- Bench, which advances VOR evaluation through three integrated components. First, we present the VOR Dataset (VORD), the first benchmark dataset providing both paired edited videos and graffiti masks. Its unique strength lies in a diverse data spectrum, which encompasses model-generated, tool-rendered, and camera-captured data, ensuring robust assessment across real-world scenarios. Second, we develop rMPAF, a realistic Motion- capable Paired-video Acquisition Framework. By combining the strengths of image- based object removal and fine-tuned video generation models, rMPAF automatically generates realistic, motion-coherent paired videos. Finally, we propose three evaluation dimensions and introduce VOR-MDSM, the first perception-driven VLM-based scoring model specifically designed for mask-guided VOR. It bridges the gap between arithmetic metrics and human perception by covering the essential visual attributes and matching nuanced human judgment. Extensive experiments demonstrate that VOR-Bench yields evaluation results that align closely with human perception, achieving a remarkable cor- relation (\r{ho} > 0.9) with subjective assessments. We will release VOR-Bench along with its documentation to ensure full reproducibility.

==> tab/ablation_scribble_masks.tex <==
\begin{table}[!t]
  \caption{Ablation study on Scribble masks. Each value in the table represents the score obtained using segmentation masks minus the score obtained using graffiti masks.}
  \label{tab:4}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{ccccc 
  }
    \toprule
    % 前4列跨行合并并居中
    \multirow{2}{*}{\centering Models} & \multicolumn{1}{c}{Removal} & \multicolumn{1}{c}{M-Bg} & \multicolumn{1}{c}{Logical} & \multirow{2}{*}{\centering Overall} \\
    & Comp. & Consist. & Plaus. &  \\
    \midrule
    ProPainter~\cite{zhou2023propainter} & -0.04 & 0.04 & 0.09 & 0.03  \\
    FloED~\cite{gu2024advanced} & 0.08 & 0.21 & 0.06 & 0.12  \\
    FGT~\cite{zhang2022flow} & 0.00 & 0.05 & -0.01 & 0.01  \\
    FuseFormer~\cite{liu2021fuseformer}  & 0.00 & 0.04 & 0.11 & 0.05  \\
    Casper~\cite{lee2025generative} & 0.04 & 0.14 & 0.17 & 0.12  \\
    DiffuEraser~\cite{li2025diffueraser} & -0.02 & 0.02 & 0.05 & 0.02  \\
    Minimax-Remover~\cite{zi2025minimax}  & 0.00  & 0.08 & 0.12 & 0.07  \\
    ROSE~\cite{miao2025rose} & 0.02  & 0.08 & 0.01 & 0.04  \\
    \bottomrule
  \end{tabular}%
  }
\end{table}

==> tab/background.tex <==
% \begin{table}[htbp]
%   \caption{Quantitative results among all comparison models on background preservation. Bold indicates the best, underlined indicates the second-best.}
%   \label{tab:bg}
%   \centering
%   \setlength{\heavyrulewidth}{0.2mm} % toprule的粗细
%   \setlength{\lightrulewidth}{0.1mm} 
%   \scriptsize
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{cccc 
%   }
%     \toprule
%     % 前4列跨行合并并居中
%     \multirow{2}{*}{\centering Models} & \multicolumn{3}{c}{Background Preservation} \\
%     \cmidrule(lr){2-4}
%     & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
%     \midrule
%     FuseFormer~\cite{liu2021fuseformer}  & 28.0921 & 0.8717 & 0.0604  \\
%     FGT~\cite{zhang2022flow} & 27.3927 & 0.8346 & 0.1084  \\
%     ProPainter~\cite{zhou2023propainter} & \underline{28.6649}& \textbf{0.8845} & \textbf{0.0522}  \\
%     FloED~\cite{gu2024advanced} & 27.2847 & 0.8743 & 0.0753  \\
%     Casper~\cite{lee2025generative} & 27.9612 & 0.8489 & 0.0645  \\
%     DiffuEraser~\cite{li2025diffueraser} & 28.4647 & \underline{0.8831} & \underline{0.0529}  \\
%     MiniMax-Remover~\cite{zi2025minimax}  & 27.7893 & 0.8579 & 0.0653  \\
%     ROSE~\cite{miao2025rose} & \textbf{28.6677} & 0.8549 & 0.0612  \\
%     \bottomrule
%   \end{tabular}%
%   }
%   \vspace{-9pt}
% \end{table}

==> tab/data_effectiveness.tex <==
% \begin{table}[t!]
%   \caption{Proof of synthetic data validity.}
%   \label{tab:data_effect}
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{threeparttable}
%   \begin{tabular}{cccccc}
%     \toprule
%     % 前4列跨行合并并居中
%     \multirow{2}{*}{\centering Models} & \multirow{2}{*}{\centering RotError $\downarrow$} & \multicolumn{2}{c}{TransError $\downarrow$} & \multicolumn{2}{c}{CamMC $\downarrow$}  \\
%     \cmidrule(lr){3-4}\cmidrule(lr){5-6}
%     &  & Rel.\tnote{*}& Abs.\tnote{*} & Rel. & Abs. \\
%     \midrule
%     Klingv1.6 & 21.68 & 48.49 & 196.14 & 62.57 & 207.65  \\
%     Wan2.1~\cite{wan2025wan} & 27.80 & 48.31 & 99.61 & 67.82 & 115.76  \\
%     \midrule
%     Ours & 0.40  & 23.48 & 64.05 & 23.62 & 64.16  \\
%     \bottomrule
%   \end{tabular}
%   \begin{tablenotes}
%         \footnotesize
%         \item[*] Rel. represents the relative score of the metric. Abs. represents the absolute score of the metric. %此处加入注释**信息
%       \end{tablenotes}
%     \end{threeparttable}
%   }
%   \vspace{-9pt}
% \end{table}

\begin{wraptable}{r}{0.5\textwidth}
  \centering
  \caption{Proof of synthetic data validity.}
  \label{tab:data_effect}

  % \resizebox{\linewidth}{!}{
  \begin{threeparttable}
  \begin{tabular}{cccccc}
    \toprule
    % 前4列跨行合并并居中
    \multirow{2}{*}{\centering Models} & \multirow{2}{*}{\centering RotError $\downarrow$} & \multicolumn{2}{c}{TransError $\downarrow$} & \multicolumn{2}{c}{CamMC $\downarrow$}  \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    &  & Rel.\tnote{*}& Abs.\tnote{*} & Rel. & Abs. \\
    \midrule
    Klingv1.6 & 21.68 & 48.49 & 196.14 & 62.57 & 207.65  \\
    Wan2.1~\cite{wan2025wan} & 27.80 & 48.31 & 99.61 & 67.82 & 115.76  \\
    \midrule
    Ours & 0.40  & 23.48 & 64.05 & 23.62 & 64.16  \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
        \footnotesize
        \item[*] Rel. represents the relative score of the metric. Abs. represents the absolute score of the metric. %此处加入注释**信息
      \end{tablenotes}
    \end{threeparttable}
  % }
  \vspace{-9pt}

\end{wraptable}

==> tab/datasets.tex <==
\begin{table}[t]
  \caption{
        A comparative analysis of existing video object removal datasets and our proposed VORD, highlighting differences in ground-truth videos, graffiti masks, and data diversity.}
  \label{tab:1}
  \centering
  \resizebox{0.85\linewidth}{!}{% 单栏适配页面宽度
  \footnotesize
  \begin{tabular}{
    >{\centering\arraybackslash}m{2.8cm}    % Dataset列
    >{\centering\arraybackslash}m{1cm}    % Size列
    >{\centering\arraybackslash}m{1.2cm}  % ground truth Videos列
    >{\centering\arraybackslash}m{1.2cm}  % scribble masks列
    >{\centering\arraybackslash}m{1.2cm}  % Synthetic列
    >{\centering\arraybackslash}m{1.2cm}  % Real列
    >{\centering\arraybackslash}m{1.2cm}  % Rendered列
  }
    \toprule
    % 前4列跨行合并并居中
    \multirow{2}{*}{\centering Dataset} & \multirow{2}{*}{\centering Size} & \multicolumn{1}{c}{Ground } & \multicolumn{1}{c}{Graffiti } & \multicolumn{3}{c}{Video Types} \\
    \cmidrule(lr){5-7}  % 仅分隔Video Types子列
    &               &       Truth       &    Masks      & Synthetic & Real & Rendered \\
    \midrule
    DAVIS~\cite{pont20172017} & 90   &  &       &  & \ding{51} &  \\
    YouTube-VOS~\cite{xu2018youtube}   & 508  &  &       &  & \ding{51} &  \\
    ROSE-Bench~\cite{miao2025rose}    & 60   & \ding{51} &       &  & & \ding{51} \\
    Movies~\cite{lin2023omnimatterf}         & 5    & \ding{51} &       &  &  & \ding{51} \\
    HQVI~\cite{cho2025elevating}          & 10   & \ding{51} &      & \ding{51} &  &  \\
    \midrule
    VORD        & 150  & \ding{51} & \ding{51}      & \ding{51} & \ding{51} & \ding{51} \\
    \bottomrule
  \end{tabular}%
  }
  \vspace{-11pt}
\end{table}

\begin{figtab}
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \includegraphics[width = \linewidth]{eccv2026_hhn/figure/old_metrics_8.pdf}
    \figcaption{Limitations of the traditional metric in reflecting whether unexpected content is generated. The bottom line shows the best removal effect yet receives the lowest SSIM score.}
    \label{fig:old_metrics}
  \end{minipage}\quad
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \tabcaption{A comparative analysis of existing video object removal datasets and our proposed VORD, highlighting differences in ground-truth videos, graffiti masks, and data diversity.}
    \label{tab:1}
    \begin{tabular}{
    >{\centering\arraybackslash}m{2.8cm}    % Dataset列
    >{\centering\arraybackslash}m{1cm}    % Size列
    >{\centering\arraybackslash}m{1.2cm}  % ground truth Videos列
    >{\centering\arraybackslash}m{1.2cm}  % scribble masks列
    >{\centering\arraybackslash}m{1.2cm}  % Synthetic列
    >{\centering\arraybackslash}m{1.2cm}  % Real列
    >{\centering\arraybackslash}m{1.2cm}  % Rendered列
  }
    \toprule
    % 前4列跨行合并并居中
    \multirow{2}{*}{\centering Dataset} & \multirow{2}{*}{\centering Size} & \multicolumn{1}{c}{Ground } & \multicolumn{1}{c}{Graffiti } & \multicolumn{3}{c}{Video Types} \\
    \cmidrule(lr){5-7}  % 仅分隔Video Types子列
    &               &       Truth       &    Masks      & Synthetic & Real & Rendered \\
    \midrule
    DAVIS~\cite{pont20172017} & 90   &  &       &  & \ding{51} &  \\
    YouTube-VOS~\cite{xu2018youtube}   & 508  &  &       &  & \ding{51} &  \\
    ROSE-Bench~\cite{miao2025rose}    & 60   & \ding{51} &       &  & & \ding{51} \\
    Movies~\cite{lin2023omnimatterf}         & 5    & \ding{51} &       &  &  & \ding{51} \\
    HQVI~\cite{cho2025elevating}          & 10   & \ding{51} &      & \ding{51} &  &  \\
    \midrule
    VORD        & 150  & \ding{51} & \ding{51}      & \ding{51} & \ding{51} & \ding{51} \\
    \bottomrule
  \end{tabular}
  \end{minipage}
\end{figtab}


==> tab/mainexperiment.tex <==
% \begin{table}[htbp]
%   \caption{Quantitative results among all comparison models across three dimensions. Bold indicates the best, underlined indicates the second-best.}
%   \label{tab:2}
%   \centering
%     % {
%   \begin{threeparttable}
%   % \Huge
%   \setlength{\heavyrulewidth}{0.8mm} % toprule的粗细
%   \setlength{\lightrulewidth}{0.5mm}
%   % \resizebox{\linewidth}{!}{
%   %\begin{tabular}{\linewidth}{@{\extracolsep{\fill}}cccccc}
%   \begin{tabular}{cccccc}
%     \toprule
%     % 前4列跨行合并并居中
%     \multirow{2}{*}{\centering Models} & \multirow{2}{*}{\centering Year} & \multicolumn{1}{c}{Removal} & \multicolumn{1}{c}{M-Bg} & \multicolumn{1}{c}{Logical} & \multirow{2}{*}{\centering Overall} \\
%     & & Comp.\tnote{*} & Consist.\tnote{*} & Plaus.\tnote{*} &   \\
%     \midrule
%     FuseFormer~\cite{liu2021fuseformer} & 2021 & 3.53 & 3.36 & 3.93 & 3.61  \\
%     FGT~\cite{zhang2022flow} & 2022 & 3.49 & 3.25 & 3.88 & 3.54 \\
%     ProPainter~\cite{zhou2023propainter} & 2023 & 3.17 & 2.85 & 3.50 & 3.17  \\
%     FloED~\cite{gu2024advanced} & 2024 & 3.15 & 3.04 & 3.43 & 3.21  \\
%     Casper~\cite{lee2025generative} & 2025 & 3.81 & 3.77 & 4.12 & 3.90  \\
%     DiffuEraser~\cite{li2025diffueraser} & 2025 & 3.76 & 3.59 & 4.12 & 3.82  \\
%     MiniMax-Remover~\cite{zi2025minimax} & 2025 & \underline{3.93}  & \underline{3.77} & \underline{4.25} & \underline{3.98}  \\
%     ROSE~\cite{miao2025rose} & 2025 & \textbf{4.33}  & \textbf{4.20} & \textbf{4.67} & \textbf{4.40}  \\
%     \bottomrule



%   \end{tabular}
%   % }
%     \begin{tablenotes}
%         \footnotesize
%         \item[*] Removal Comp.: Object Removal Completeness; \\ M-Bg Consist.: Mask-Background Consistency; \\ Logical Plaus.: Logical Plausibility.  %此处加入注释*信息
%       \end{tablenotes}
%       \end{threeparttable}

  
% \end{table}

\begin{table*}[t] % table* 跨双栏
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \caption{Quantitative results among all comparison models across three dimensions. Bold indicates the best, underlined indicates the second-best.}
        \label{tab:2}
        \centering
        % {
        \begin{threeparttable}
        % \Huge
        \setlength{\heavyrulewidth}{0.8mm} % toprule的粗细
        \setlength{\lightrulewidth}{0.5mm}
        % \resizebox{\linewidth}{!}{
        %\begin{tabular}{\linewidth}{@{\extracolsep{\fill}}cccccc}
        \begin{tabular}{cccccc}
            \toprule
            % 前4列跨行合并并居中
            \multirow{2}{*}{\centering Models} & \multirow{2}{*}{\centering Year} & \multicolumn{1}{c}{Removal} & \multicolumn{1}{c}{M-Bg} & \multicolumn{1}{c}{Logical} & \multirow{2}{*}{\centering Overall} \\
            & & Comp.\tnote{*} & Consist.\tnote{*} & Plaus.\tnote{*} &   \\
             \midrule
            FuseFormer~\cite{liu2021fuseformer} & 2021 & 3.53 & 3.36 & 3.93 & 3.61  \\
            FGT~\cite{zhang2022flow} & 2022 & 3.49 & 3.25 & 3.88 & 3.54 \\
            ProPainter~\cite{zhou2023propainter} & 2023 & 3.17 & 2.85 & 3.50 & 3.17  \\
            FloED~\cite{gu2024advanced} & 2024 & 3.15 & 3.04 & 3.43 & 3.21  \\
            Casper~\cite{lee2025generative} & 2025 & 3.81 & 3.77 & 4.12 & 3.90  \\
            DiffuEraser~\cite{li2025diffueraser} & 2025 & 3.76 & 3.59 & 4.12 & 3.82  \\
            MiniMax-Remover~\cite{zi2025minimax} & 2025 & \underline{3.93}  & \underline{3.77} & \underline{4.25} & \underline{3.98}  \\
            ROSE~\cite{miao2025rose} & 2025 & \textbf{4.33}  & \textbf{4.20} & \textbf{4.67} & \textbf{4.40}  \\
            \bottomrule
        \end{tabular}
  % }
        \begin{tablenotes}
            \footnotesize
            \item[*] Removal Comp.: Object Removal Completeness; \\ M-Bg Consist.: Mask-Background Consistency; \\ Logical Plaus.: Logical Plausibility.  %此处加入注释*信息
        \end{tablenotes}
        \end{threeparttable}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \caption{Quantitative results among all comparison models on background preservation. Bold indicates the best, underlined indicates the second-best.}
        \label{tab:bg}
        \centering
        \setlength{\heavyrulewidth}{0.2mm} % toprule的粗细
        \setlength{\lightrulewidth}{0.1mm} 
        \scriptsize
        % \resizebox{\linewidth}{!}{
        \begin{tabular}{cccc }
            \toprule
            % 前4列跨行合并并居中
            \multirow{2}{*}{\centering Models} & \multicolumn{3}{c}{Background Preservation} \\
            \cmidrule(lr){2-4}
            & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
            \midrule
            FuseFormer~\cite{liu2021fuseformer}  & 28.0921 & 0.8717 & 0.0604  \\
            FGT~\cite{zhang2022flow} & 27.3927 & 0.8346 & 0.1084  \\
            ProPainter~\cite{zhou2023propainter} & \underline{28.6649}& \textbf{0.8845} & \textbf{0.0522}  \\
            FloED~\cite{gu2024advanced} & 27.2847 & 0.8743 & 0.0753  \\
            Casper~\cite{lee2025generative} & 27.9612 & 0.8489 & 0.0645  \\
            DiffuEraser~\cite{li2025diffueraser} & 28.4647 & \underline{0.8831} & \underline{0.0529}  \\
            MiniMax-Remover~\cite{zi2025minimax}  & 27.7893 & 0.8579 & 0.0653  \\
            ROSE~\cite{miao2025rose} & \textbf{28.6677} & 0.8549 & 0.0612  \\
            \bottomrule
        \end{tabular}%
        % }
        \vspace{-9pt}
    \end{minipage}
\end{table*}


